New Harmonic Coils for Enhanced Beam Extraction at the U-120M Cyclotron

Since its commissioning in 1977, the U-120M cyclotron has been equipped with one pair of harmonic coils dedicated to establishing optimal beam quality at low accelerating radii. In 2022, the cyclotron was upgraded and a second pair of harmonic coils was added. The new harmonic coils are positioned at a radius of approximately 50\,cm corresponding to the outermost beam orbit, where they were installed to ensure efficient extraction of positively accelerated ions from the cyclotron in the newly developed extraction system. This article describes in detail the design of the new harmonic coils, their installation in the accelerator vacuum chamber, and their use in the extraction process. Furthermore, the design of a new extraction system using the precession and linear integer resonance extraction methods is presented and a comparison of the basic properties of these two methods is given. Finally, an evaluation of their advantages and limitations concerning their possible use in the cyclotron and an estimation of the efficiency of the new extraction system is made.

==> intro2.tex <==
The U-120M cyclotron, located at the Nuclear Physics Institute in Rez, near Prague, is a warm-magnet, multi-particle, wide-energy-range isochronous cyclotron. Established in 1976, this cyclotron boasts a K-value of up to 40 MeV. It's designed to accelerate particles with a mass-to-charge ratio (A/Z) of 2 or lower.

The cyclotron has a magnet pole diameter of 60 cm. It's capable of accelerating helium-3 ($^3$He) to 55 MeV, alpha particles to 40 MeV, and both protons and deuterons to 40 MeV. Moreover, it can achieve intensities of several tens of microamperes.

The U-120M can operate to accelerate both positive and negative ions, thanks to its internal PIG-type ion source. For a more detailed overview of the cyclotron facility, readers are referred to the source  \cite{filip_irad_setup}. 






